Patient-Oriented Unsupervised Learning to Unlock Patterns of Multimorbidity Associated with Stroke using Primary Care Electronic Health Records

Background: Identifying and characterising the longitudinal patterns of multimorbidity associated with stroke is needed to better understand patients' needs and inform new models of care. Methods: We used an unsupervised patient-oriented clustering approach to analyse primary care electronic health records (EHR) of 30 common long-term conditions (LTC), in patients with stroke aged over 18, registered in 41 general practices in south London between 2005 and 2021. Results: Of 849,968 registered patients, 9,847 (1.16%) had a record of stroke, 46.5% were female and median age at record was 65.0 year (IQR: 51.5 to 77.0). The median number of LTCs in addition to stroke was 3 (IQR: from 2 to 5). Patients were stratified in eight clusters. These clusters revealed contrasted patterns of multimorbidity, socio-demographic characteristics (age, gender and ethnicity) and risk factors. Beside a core of 3 clusters associated with conventional stroke risk-factors, minor clusters exhibited less common but recurrent combinations of LTCs including mental health conditions, asthma, osteoarthritis and sickle cell anaemia. Importantly, complex profiles combining mental health conditions, infectious diseases and substance dependency emerged. Conclusion: This patient-oriented approach to EHRs uncovers the heterogeneity of profiles of multimorbidity and socio-demographic characteristics associated with stroke. It highlights the importance of conventional stroke risk factors as well as the association of mental health conditions in complex profiles of multimorbidity displayed in a significant proportion of patients. These results address the need for a better understanding of stroke-associated multimorbidity and complexity to inform more efficient and patient-oriented healthcare models.

==> tab1.tex <==

\begin{landscape}\begingroup\fontsize{8}{10}\selectfont

\begin{longtable}[t]{lllllllllll}
\caption{\label{tab:t1}Distribution of the 30 analysed long-term conditions across defined clusters}\\
\toprule
Cluster \# & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Total & P\\
\midrule
\endfirsthead
\caption[]{Distribution of the 30 analysed long-term conditions across defined clusters \textit{(continued)}}\\
\toprule
Cluster \# & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Total & P\\
\midrule
\endhead
\midrule
\multicolumn{11}{r@{}}{\textit{(Continued on Next Page...)}}\
\endfoot
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\textsuperscript{a} Chronic Obstructive Pulmonary Disease}\\
\multicolumn{11}{l}{\rule{0pt}{1em}\textsuperscript{b} Human Immunodeficiency Virus/Acquired Immunodeficiency Syndrome}\\
\multicolumn{11}{l}{\rule{0pt}{1em}\textsuperscript{c} Chronic Kidney Disease stage 3 to stage 5}\\
\multicolumn{11}{l}{\rule{0pt}{1em}\textsuperscript{d} Transient Ischemic Attack}\\
\endlastfoot
\cellcolor{gray!6}{Coronary Heart Disease} & \cellcolor{gray!6}{419 (17.5)} & \cellcolor{gray!6}{335 (18.5)} & \cellcolor{gray!6}{382 (21.4)} & \cellcolor{gray!6}{267 (18.9)} & \cellcolor{gray!6}{84 (9.9)} & \cellcolor{gray!6}{140 (20.4)} & \cellcolor{gray!6}{10 (1.8)} & \cellcolor{gray!6}{19 (5.3)} & \cellcolor{gray!6}{1656 (16.8)} & \cellcolor{gray!6}{<0.001}\\
Parkinson's disease & 61 (2.6) & 58 (3.2) & 39 (2.2) & 16 (1.1) & 5 (0.6) & 17 (2.5) & 0 (0.0) & 2 (0.6) & 198 (2.0) & <0.001\\
\cellcolor{gray!6}{Heart Failure} & \cellcolor{gray!6}{296 (12.4)} & \cellcolor{gray!6}{264 (14.6)} & \cellcolor{gray!6}{278 (15.6)} & \cellcolor{gray!6}{190 (13.5)} & \cellcolor{gray!6}{63 (7.5)} & \cellcolor{gray!6}{113 (16.5)} & \cellcolor{gray!6}{12 (2.1)} & \cellcolor{gray!6}{7 (2.0)} & \cellcolor{gray!6}{1223 (12.4)} & \cellcolor{gray!6}{<0.001}\\
Osteoarthritis & 566 (23.7) & 401 (22.1) & 421 (23.6) & 324 (23.0) & 138 (16.3) & 683 (99.7) & 26 (4.6) & 24 (6.7) & 2583 (26.2) & <0.001\\
\cellcolor{gray!6}{Asthma} & \cellcolor{gray!6}{441 (18.4)} & \cellcolor{gray!6}{244 (13.5)} & \cellcolor{gray!6}{79 (4.4)} & \cellcolor{gray!6}{72 (5.1)} & \cellcolor{gray!6}{342 (40.5)} & \cellcolor{gray!6}{38 (5.5)} & \cellcolor{gray!6}{27 (4.8)} & \cellcolor{gray!6}{12 (3.4)} & \cellcolor{gray!6}{1255 (12.7)} & \cellcolor{gray!6}{<0.001}\\
Serious Mental Illness & 280 (11.7) & 50 (2.8) & 26 (1.5) & 32 (2.3) & 46 (5.4) & 2 (0.3) & 16 (2.8) & 7 (2.0) & 459 (4.7) & <0.001\\
\cellcolor{gray!6}{Hypertension} & \cellcolor{gray!6}{1430 (59.8)} & \cellcolor{gray!6}{1206 (66.5)} & \cellcolor{gray!6}{1424 (79.9)} & \cellcolor{gray!6}{1301 (92.3)} & \cellcolor{gray!6}{352 (41.7)} & \cellcolor{gray!6}{485 (70.8)} & \cellcolor{gray!6}{64 (11.4)} & \cellcolor{gray!6}{82 (23.0)} & \cellcolor{gray!6}{6344 (64.4)} & \cellcolor{gray!6}{<0.001}\\
Depression & 844 (35.3) & 317 (17.5) & 200 (11.2) & 274 (19.4) & 531 (62.8) & 84 (12.3) & 64 (11.4) & 26 (7.3) & 2340 (23.8) & <0.001\\
\cellcolor{gray!6}{Anxiety Disorders} & \cellcolor{gray!6}{517 (21.6)} & \cellcolor{gray!6}{329 (18.1)} & \cellcolor{gray!6}{146 (8.2)} & \cellcolor{gray!6}{233 (16.5)} & \cellcolor{gray!6}{570 (67.5)} & \cellcolor{gray!6}{91 (13.3)} & \cellcolor{gray!6}{79 (14.0)} & \cellcolor{gray!6}{23 (6.4)} & \cellcolor{gray!6}{1988 (20.2)} & \cellcolor{gray!6}{<0.001}\\
Cancer & 460 (19.2) & 387 (21.3) & 351 (19.7) & 133 (9.4) & 85 (10.1) & 88 (12.8) & 9 (1.6) & 25 (7.0) & 1538 (15.6) & <0.001\\
\cellcolor{gray!6}{Peripheral Aterial/Vascular Disease} & \cellcolor{gray!6}{169 (7.1)} & \cellcolor{gray!6}{111 (6.1)} & \cellcolor{gray!6}{181 (10.2)} & \cellcolor{gray!6}{113 (8.0)} & \cellcolor{gray!6}{25 (3.0)} & \cellcolor{gray!6}{52 (7.6)} & \cellcolor{gray!6}{1 (0.2)} & \cellcolor{gray!6}{1 (0.3)} & \cellcolor{gray!6}{653 (6.6)} & \cellcolor{gray!6}{<0.001}\\
Diabetes & 626 (26.2) & 409 (22.5) & 710 (39.8) & 831 (59.0) & 177 (20.9) & 190 (27.7) & 26 (4.6) & 37 (10.4) & 3006 (30.5) & <0.001\\
\cellcolor{gray!6}{Chronic Kidney Disease Stage 3-5} & \cellcolor{gray!6}{444 (18.6)} & \cellcolor{gray!6}{514 (28.3)} & \cellcolor{gray!6}{565 (31.7)} & \cellcolor{gray!6}{423 (30.0)} & \cellcolor{gray!6}{107 (12.7)} & \cellcolor{gray!6}{207 (30.2)} & \cellcolor{gray!6}{22 (3.9)} & \cellcolor{gray!6}{14 (3.9)} & \cellcolor{gray!6}{2296 (23.3)} & \cellcolor{gray!6}{<0.001}\\
Viral Hepatitis (B\&C) & 105 (4.4) & 10 (0.6) & 9 (0.5) & 21 (1.5) & 23 (2.7) & 6 (0.9) & 6 (1.1) & 5 (1.4) & 185 (1.9) & <0.001\\
\cellcolor{gray!6}{Inflammatory Bowel Disease} & \cellcolor{gray!6}{58 (2.4)} & \cellcolor{gray!6}{23 (1.3)} & \cellcolor{gray!6}{16 (0.9)} & \cellcolor{gray!6}{18 (1.3)} & \cellcolor{gray!6}{19 (2.2)} & \cellcolor{gray!6}{14 (2.0)} & \cellcolor{gray!6}{4 (0.7)} & \cellcolor{gray!6}{1 (0.3)} & \cellcolor{gray!6}{153 (1.6)} & \cellcolor{gray!6}{<0.001}\\
Liver Disease & 99 (4.1) & 17 (0.9) & 14 (0.8) & 22 (1.6) & 37 (4.4) & 6 (0.9) & 3 (0.5) & 1 (0.3) & 199 (2.0) & <0.001\\
\cellcolor{gray!6}{Epilepsy} & \cellcolor{gray!6}{378 (15.8)} & \cellcolor{gray!6}{58 (3.2)} & \cellcolor{gray!6}{61 (3.4)} & \cellcolor{gray!6}{66 (4.7)} & \cellcolor{gray!6}{71 (8.4)} & \cellcolor{gray!6}{38 (5.5)} & \cellcolor{gray!6}{46 (8.2)} & \cellcolor{gray!6}{14 (3.9)} & \cellcolor{gray!6}{732 (7.4)} & \cellcolor{gray!6}{<0.001}\\
Osteopotosis & 94 (3.9) & 206 (11.4) & 118 (6.6) & 29 (2.1) & 23 (2.7) & 67 (9.8) & 2 (0.4) & 5 (1.4) & 544 (5.5) & <0.001\\
\cellcolor{gray!6}{Dementia/Alzheimer's} & \cellcolor{gray!6}{277 (11.6)} & \cellcolor{gray!6}{460 (25.4)} & \cellcolor{gray!6}{352 (19.8)} & \cellcolor{gray!6}{132 (9.4)} & \cellcolor{gray!6}{42 (5.0)} & \cellcolor{gray!6}{172 (25.1)} & \cellcolor{gray!6}{4 (0.7)} & \cellcolor{gray!6}{12 (3.4)} & \cellcolor{gray!6}{1451 (14.7)} & \cellcolor{gray!6}{<0.001}\\
Sickle Cell Anaemia & 11 (0.5) & 1 (0.1) & 1 (0.1) & 3 (0.2) & 2 (0.2) & 1 (0.1) & 41 (7.3) & 0 (0.0) & 60 (0.6) & <0.001\\
\cellcolor{gray!6}{Multiple Sclerosis} & \cellcolor{gray!6}{12 (0.5)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{1 (0.1)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{7 (0.8)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{2 (0.4)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{22 (0.2)} & \cellcolor{gray!6}{<0.001}\\
HIV/AIDS\textsuperscript{b} & 85 (3.6) & 1 (0.1) & 3 (0.2) & 10 (0.7) & 11 (1.3) & 0 (0.0) & 2 (0.4) & 1 (0.3) & 113 (1.1) & <0.001\\
\cellcolor{gray!6}{Myocardial infarction} & \cellcolor{gray!6}{222 (9.3)} & \cellcolor{gray!6}{163 (9.0)} & \cellcolor{gray!6}{238 (13.4)} & \cellcolor{gray!6}{127 (9.0)} & \cellcolor{gray!6}{48 (5.7)} & \cellcolor{gray!6}{66 (9.6)} & \cellcolor{gray!6}{8 (1.4)} & \cellcolor{gray!6}{7 (2.0)} & \cellcolor{gray!6}{879 (8.9)} & \cellcolor{gray!6}{<0.001}\\
Atrial Fibrillation & 365 (15.3) & 491 (27.1) & 388 (21.8) & 141 (10.0) & 74 (8.8) & 184 (26.9) & 13 (2.3) & 16 (4.5) & 1672 (17.0) & <0.001\\
\cellcolor{gray!6}{Lupus} & \cellcolor{gray!6}{34 (1.4)} & \cellcolor{gray!6}{1 (0.1)} & \cellcolor{gray!6}{4 (0.2)} & \cellcolor{gray!6}{4 (0.3)} & \cellcolor{gray!6}{7 (0.8)} & \cellcolor{gray!6}{1 (0.1)} & \cellcolor{gray!6}{1 (0.2)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{52 (0.5)} & \cellcolor{gray!6}{<0.001}\\
Chronic Obstructive Pulmonary Disease & 337 (14.1) & 249 (13.7) & 152 (8.5) & 60 (4.3) & 85 (10.1) & 54 (7.9) & 9 (1.6) & 8 (2.2) & 954 (9.7) & <0.001\\
\cellcolor{gray!6}{Rheumatoid Arthritis} & \cellcolor{gray!6}{89 (3.7)} & \cellcolor{gray!6}{29 (1.6)} & \cellcolor{gray!6}{19 (1.1)} & \cellcolor{gray!6}{29 (2.1)} & \cellcolor{gray!6}{15 (1.8)} & \cellcolor{gray!6}{21 (3.1)} & \cellcolor{gray!6}{2 (0.4)} & \cellcolor{gray!6}{1 (0.3)} & \cellcolor{gray!6}{205 (2.1)} & \cellcolor{gray!6}{<0.001}\\
Transient Ischemic Attack & 443 (18.5) & 283 (15.6) & 425 (23.8) & 165 (11.7) & 109 (12.9) & 111 (16.2) & 12 (2.1) & 9 (2.5) & 1557 (15.8) & <0.001\\
\cellcolor{gray!6}{Cognitive and learning disability} & \cellcolor{gray!6}{49 (2.0)} & \cellcolor{gray!6}{2 (0.1)} & \cellcolor{gray!6}{3 (0.2)} & \cellcolor{gray!6}{9 (0.6)} & \cellcolor{gray!6}{9 (1.1)} & \cellcolor{gray!6}{2 (0.3)} & \cellcolor{gray!6}{11 (2.0)} & \cellcolor{gray!6}{0 (0.0)} & \cellcolor{gray!6}{85 (0.9)} & \cellcolor{gray!6}{<0.001}\\
Total N (\%) & 2392 (24.3) & 1814 (18.4) & 1782 (18.1) & 1409 (14.3) & 845 (8.6) & 685 (7.0) & 563 (5.7) & 357 (3.6) & 9847 & \\*
\end{longtable}
\endgroup{}
\end{landscape}



==> tab2.tex <==

\begin{landscape}\begingroup\fontsize{6}{8}\selectfont

\begin{longtable}[t]{llllllllllll}
\caption{\label{tab:t2}Distribution of socio-demographics and risk factors associated to stroke accross the clusters}\\
\toprule
Cluster \# &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Total & P\\
\midrule
\endfirsthead
\caption[]{Distribution of socio-demographics and risk factors associated to stroke accross the clusters \textit{(continued)}}\\
\toprule
Cluster \# &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Total & P\\
\midrule
\endhead
\midrule
\multicolumn{12}{r@{}}{\textit{(Continued on Next Page...)}}\
\endfoot
\bottomrule
\multicolumn{12}{l}{\rule{0pt}{1em}\textsuperscript{a} IMD\textsuperscript{a} quitile 1 (most deprived)-2 vs 3-5 (less deprived)}\\
\multicolumn{12}{l}{\rule{0pt}{1em}\textsuperscript{b} Long-term condition}\\
\endlastfoot
\cellcolor{gray!6}{Gender} & \cellcolor{gray!6}{Female} & \cellcolor{gray!6}{1025 (42.9)} & \cellcolor{gray!6}{969 (53.4)} & \cellcolor{gray!6}{729 (40.9)} & \cellcolor{gray!6}{581 (41.2)} & \cellcolor{gray!6}{463 (54.8)} & \cellcolor{gray!6}{404 (59.0)} & \cellcolor{gray!6}{271 (48.1)} & \cellcolor{gray!6}{133 (37.3)} & \cellcolor{gray!6}{4575 (46.5)} & \cellcolor{gray!6}{<0.001}\\
Age at onset & Median (IQR) & 59.2 (52.6 to 68.0) & 81.2 (76.1 to 86.3) & 70.7 (65.8 to 77.0) & 55.0 (49.0 to 63.0) & 47.0 (36.0 to 56.9) & 78.1 (69.5 to 85.4) & 26.8 (19.2 to 32.0) & 44.4 (41.1 to 47.0) & 65.0 (51.5 to 77.0) & <0.001\\
\cellcolor{gray!6}{Ethnicity} & \cellcolor{gray!6}{White} & \cellcolor{gray!6}{1284 (53.7)} & \cellcolor{gray!6}{1088 (60.0)} & \cellcolor{gray!6}{830 (46.6)} & \cellcolor{gray!6}{441 (31.3)} & \cellcolor{gray!6}{497 (58.8)} & \cellcolor{gray!6}{361 (52.7)} & \cellcolor{gray!6}{307 (54.5)} & \cellcolor{gray!6}{191 (53.5)} & \cellcolor{gray!6}{4999 (50.8)} & \cellcolor{gray!6}{<0.001}\\
 & Asian & 147 (6.1) & 103 (5.7) & 138 (7.7) & 131 (9.3) & 42 (5.0) & 43 (6.3) & 21 (3.7) & 20 (5.6) & 645 (6.6) & \\
\cellcolor{gray!6}{} & \cellcolor{gray!6}{Black} & \cellcolor{gray!6}{550 (23.0)} & \cellcolor{gray!6}{268 (14.8)} & \cellcolor{gray!6}{485 (27.2)} & \cellcolor{gray!6}{619 (43.9)} & \cellcolor{gray!6}{185 (21.9)} & \cellcolor{gray!6}{168 (24.5)} & \cellcolor{gray!6}{128 (22.7)} & \cellcolor{gray!6}{92 (25.8)} & \cellcolor{gray!6}{2495 (25.3)} & \cellcolor{gray!6}{}\\
 & Mixed & 78 (3.3) & 33 (1.8) & 54 (3.0) & 52 (3.7) & 32 (3.8) & 20 (2.9) & 30 (5.3) & 14 (3.9) & 313 (3.2) & \\
\cellcolor{gray!6}{} & \cellcolor{gray!6}{Other/Unknown} & \cellcolor{gray!6}{333 (13.9)} & \cellcolor{gray!6}{322 (17.8)} & \cellcolor{gray!6}{275 (15.4)} & \cellcolor{gray!6}{166 (11.8)} & \cellcolor{gray!6}{89 (10.5)} & \cellcolor{gray!6}{93 (13.6)} & \cellcolor{gray!6}{77 (13.7)} & \cellcolor{gray!6}{40 (11.2)} & \cellcolor{gray!6}{1395 (14.2)} & \cellcolor{gray!6}{}\\
 & <3 - Most deprived & 1638 (68.5) & 1190 (65.6) & 1192 (66.9) & 1038 (73.7) & 568 (67.2) & 451 (65.8) & 372 (66.1) & 232 (65.0) & 6681 (67.8) & <0.001\\
\cellcolor{gray!6}{IMD quintile} & \cellcolor{gray!6}{>2 - Least deprived} & \cellcolor{gray!6}{736 (30.8)} & \cellcolor{gray!6}{611 (33.7)} & \cellcolor{gray!6}{579 (32.5)} & \cellcolor{gray!6}{366 (26.0)} & \cellcolor{gray!6}{270 (32.0)} & \cellcolor{gray!6}{228 (33.3)} & \cellcolor{gray!6}{182 (32.3)} & \cellcolor{gray!6}{116 (32.5)} & \cellcolor{gray!6}{3088 (31.4)} & \cellcolor{gray!6}{}\\
 & (Missing) & 18 (0.8) & 13 (0.7) & 11 (0.6) & 5 (0.4) & 7 (0.8) & 6 (0.9) & 9 (1.6) & 9 (2.5) & 78 (0.8) & \\
\cellcolor{gray!6}{Smoking ever} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{1610 (67.3)} & \cellcolor{gray!6}{1044 (57.6)} & \cellcolor{gray!6}{1059 (59.4)} & \cellcolor{gray!6}{850 (60.3)} & \cellcolor{gray!6}{588 (69.6)} & \cellcolor{gray!6}{378 (55.2)} & \cellcolor{gray!6}{261 (46.4)} & \cellcolor{gray!6}{210 (58.8)} & \cellcolor{gray!6}{6000 (60.9)} & \cellcolor{gray!6}{<0.001}\\
Substance dependancy & 1 & 215 (9.0) & 39 (2.1) & 43 (2.4) & 57 (4.0) & 177 (20.9) & 22 (3.2) & 38 (6.7) & 18 (5.0) & 609 (6.2) & <0.001\\
\cellcolor{gray!6}{Alcohol dependence} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{744 (31.1)} & \cellcolor{gray!6}{330 (18.2)} & \cellcolor{gray!6}{416 (23.3)} & \cellcolor{gray!6}{326 (23.1)} & \cellcolor{gray!6}{296 (35.0)} & \cellcolor{gray!6}{151 (22.0)} & \cellcolor{gray!6}{94 (16.7)} & \cellcolor{gray!6}{88 (24.6)} & \cellcolor{gray!6}{2445 (24.8)} & \cellcolor{gray!6}{<0.001}\\
Chronic pain & 1 & 1440 (60.2) & 1060 (58.4) & 988 (55.4) & 810 (57.5) & 521 (61.7) & 589 (86.0) & 104 (18.5) & 90 (25.2) & 5602 (56.9) & <0.001\\
\cellcolor{gray!6}{Hypercholesterolemia} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{1738 (72.7)} & \cellcolor{gray!6}{1248 (68.8)} & \cellcolor{gray!6}{1342 (75.3)} & \cellcolor{gray!6}{1100 (78.1)} & \cellcolor{gray!6}{537 (63.6)} & \cellcolor{gray!6}{517 (75.5)} & \cellcolor{gray!6}{136 (24.2)} & \cellcolor{gray!6}{195 (54.6)} & \cellcolor{gray!6}{6813 (69.2)} & \cellcolor{gray!6}{<0.001}\\
Morbid obesity & 1 & 156 (6.5) & 51 (2.8) & 90 (5.1) & 177 (12.6) & 94 (11.1) & 46 (6.7) & 11 (2.0) & 12 (3.4) & 637 (6.5) & <0.001\\
\cellcolor{gray!6}{No. LTC\textsuperscript{b}} & \cellcolor{gray!6}{Median (IQR)} & \cellcolor{gray!6}{4.0 (2.0 to 5.0)} & \cellcolor{gray!6}{3.0 (2.0 to 5.0)} & \cellcolor{gray!6}{3.0 (2.0 to 5.0)} & \cellcolor{gray!6}{3.0 (2.0 to 5.0)} & \cellcolor{gray!6}{3.0 (2.0 to 5.0)} & \cellcolor{gray!6}{4.0 (3.0 to 5.0)} & \cellcolor{gray!6}{0.0 (0.0 to 1.0)} & \cellcolor{gray!6}{0.0 (0.0 to 1.0)} & \cellcolor{gray!6}{3.0 (2.0 to 5.0)} & \cellcolor{gray!6}{<0.001}\\
Total N (\%) &  & 2392 (24.3) & 1814 (18.4) & 1782 (18.1) & 1409 (14.3) & 845 (8.6) & 685 (7.0) & 563 (5.7) & 357 (3.6) & 9847 & \\*
\end{longtable}
\endgroup{}
\end{landscape}


